Machine Learning-Driven Open-Source Framework for Assessing QoE in Multimedia Networks

The Internet is integral to modern life, influencing communication, business, and lifestyles globally. As dependence on Internet services grows, the demand for high-quality service delivery increases. Service providers must maintain high standards of quality of service and quality of experience (QoE) to ensure user satisfaction. QoE, which reflects user satisfaction with service quality, is a key metric for multimedia services, yet it is challenging to measure due to its subjective nature and the complexities of real-time feedback. This paper introduces a machine learning-based framework for objectively assessing QoE in multimedia networks. The open-source framework complies with the ITU-T P.1203 standard. It automates data collection and user satisfaction prediction using key network parameters such as delay, jitter, packet loss, bitrate, and throughput. Using a dataset of over 20,000 records from various network conditions, the Random Forest model predicts the mean opinion score with 95.8% accuracy. Our framework addresses the limitations of existing QoE models by integrating real-time data collection, machine learning predictions, and adherence to international standards. This approach enhances QoE evaluation accuracy and allows dynamic network resource management, optimizing performance and cost-efficiency. Its open-source nature encourages adaptation and extension for various multimedia services. The findings significantly affect the telecommunications industry in managing and optimizing multimedia services. The network centric QoE prediction of the framework offers a scalable solution to improve user satisfaction without the need for content-specific data. Future enhancements could include advanced machine learning models and broader applicability to digital services. This research contributes a practical, standardized tool for QoE assessment across diverse networks and platforms.

==> abbr.tex <==
\newacronym{ACR}{ACR}{Absolute Category Rating}
\newacronym{AI}{AI}{Artificial Intelligence}
\newacronym{ANSI}{ANSI}{American National Standards Institute}
\newacronym{ANSNR}{ANSNR}{anti-noise signal-to-noise ratio}
\newacronym{BRISQUE}{BRISQUE}{Blind/referenceless image spatial quality evaluator}
\newacronym{CDN}{CDN}{Content delivery network}
\newacronym{CINR}{CINR}{Carrier to Interference and Noise Ratio}
\newacronym{DASH}{DASH}{Dynamic Adaptive Streaming over HTTP}
\newacronym{DCR}{DCR}{Degradation Category Rating}
\newacronym{DLM}{DLM}{Detail Loss Measure}
\newacronym{DSIS}{DSIS}{Double Stimulus Impairment Scale}
\newacronym{FR}{FR}{Full Reference}
\newacronym{GSM}{GSM}{Gaussian scale mixture}
\newacronym{HAR}{HAR}{HTTP Archive format}
\newacronym{HAS}{HAS}{HTTP Adaptive Streaming}
\newacronym{HTTP}{HTTP}{Hypertext Transfer Protocol}
\newacronym{HVS}{HVS}{Human visual system}
\newacronym{IF}{IF}{Influencing Factor}
\newacronym{IPTV}{IPTV}{Internet Protocol television}
\newacronym{JSON}{JSON}{JavaScript Object Notation}
\newacronym{LoM}{LoM}{level of motion}
\newacronym{LTE}{LTE}{Long-Term Evolution}
\newacronym{MI}{MI}{Motion Intensity}
\newacronym{ML}{ML}{Machine Learning}
\newacronym{MNO}{MNO}{Mobile Network Operators}
\newacronym{MOS}{MOS}{Mean Opinion Score}
\newacronym{MOVIE}{MOVIE}{Motion-based video integrity evaluation}
\newacronym{MPD}{MPD}{Media Presentation Description}
\newacronym{MPEG}{MPEG}{Moving Picture Experts Group}
\newacronym{MPQM}{MPQM}{Moving picture quality measure}
\newacronym{MS-SSIM}{MS-SSIM}{Multi-Scale structural similarity index}
\newacronym{MSE}{MSE}{Mean Squared Error}
\newacronym{NIQE}{NIQE}{Natural image quality evaluator}
\newacronym{NRP}{NRP}{No Reference  pixel-based}
\newacronym{NR}{NR}{No Reference}
\newacronym{NSS}{NSS}{natural scene statistic}
\newacronym{OTT}{OTT}{over-the-top}
\newacronym{PEVQ}{PEVQ}{Perceptual Evaluation of Video Quality}
\newacronym{PIQE}{PIQE}{Psychovisually-based image quality evaluator}
\newacronym{PI}{PI}{Pause Intensity}
\newacronym{PLR}{PLR}{Packet Loss Rate}
\newacronym{PSNR}{PSNR}{Peak signal-to-noise ratio}
\newacronym{QoE}{QoE}{Quality of Experience}
\newacronym{QoS}{QoS}{Quality of Service}
\newacronym{QP}{QP}{Quantization parameter}
\newacronym{Res}{Res}{Resolution}
\newacronym{RR}{RR}{Reduced Reference}
\newacronym{RSRP}{RSRP}{Reference Signal Received Power}
\newacronym{RSRQ}{RSRQ}{Reference Signal Received Quality}
\newacronym{RSSI}{RSSI}{Received Signal Strength Indicator}
\newacronym{RSVP}{RSVP}{Resource Reservation Protocol}
\newacronym{RTP}{RTP}{Real-time Transport Protocol}
\newacronym{SAMVIQ}{SAMVIQ}{Subjective assessment methodology for video quality}
\newacronym{SC}{SC}{Scene complexity}
\newacronym{SDSCE}{SDSCE}{Simultaneous Double Stimulus for Continuous Evaluation}
\newacronym{SINR}{SINR}{Signal to Interference and Noise Ratio}
\newacronym{SI}{SI}{Spatial Information}
\newacronym{SLA}{SLA}{service-level agreement}
\newacronym{SpEED-QA}{SpEED-QA}{Spatial efficient entropic differencing for quality assessment}
\newacronym{SSIM}{SSIM}{Structural similarity index}
\newacronym{SS}{SS}{Single stimulus}
\newacronym{STRRED}{STRRED}{Spatio-temporal reduced-reference entropic differencing}
\newacronym{SVR}{SVR}{Support Vector Regression}
\newacronym{TCP}{TCP}{Transmission Control Protocol}
\newacronym{TI}{TI}{Temporal Information}
\newacronym{ts}{ts}{Transport Stream}
\newacronym{UHD}{UHD}{Ultra High Definition}
\newacronym{VIF}{VIF}{Visual information fidelity}
\newacronym{ViLTE}{ViLTE}{Video over LTE}
\newacronym{VMAF}{VMAF}{Video multimethod assessment fusion}
\newacronym{VoD}{VoD}{video-on-demand}
\newacronym{VoIP}{VoIP}{Voice-over-Internet protocol}
\newacronym{VQA2}{VQA}{Visual Quality Assessment}
\newacronym{VQA}{VQA}{Video Quality Assessment}
\newacronym{VQM}{VQM}{Video Quality Models}
\newacronym{VSNR}{VSNR}{Visual signal-to-noise ratio}
\newacronym{ITUD}{ITU-D}{ITU Development}
\newacronym{ITUR}{ITU-R}{ITU Radiocommunication}
\newacronym{ITUT}{ITU-T}{ITU Standardization}
\newacronym{MAE}{MAE}{Mean Absolute Error}
\newacronym{RMSE}{RMSE}{Root Mean Squared Error }
\newacronym{RAE}{RAE}{Relative Absolute Error}
\newacronym{RSE}{RSE}{Relative Squared Error }
\newacronym{RDA}{RDA}{Rate Determination Algorithm}
\newacronym{SWG}{SWG}{Send While Get}
\newacronym{GBS}{GBS}{Get Before Send}
\newacronym{PRTG}{PRTG}{Paessler Router Traffic Grapher}
\newacronym{Regex}{Regex}{Regular expression}
\newacronym{bps}{bps}{bit per second}
\newacronym{kbps}{kbps}{kilobit per second}
\newacronym{ms}{ms}{millisecond}
